Performance Bounds for Expander-based Compressed Sensing in the presence of Poisson Noise

This paper provides performance bounds for compressed sensing in the presence of Poisson noise using expander graphs. The Poisson noise model is appropriate for a variety of applications, including low-light imaging and digital streaming, where the signal-independent and/or bounded noise models used in the compressed sensing literature are no longer applicable. In this paper, we develop a novel sensing paradigm based on expander graphs and propose a MAP algorithm for recovering sparse or compressible signals from Poisson observations. The geometry of the expander graphs and the positivity of the corresponding sensing matrices play a crucial role in establishing the bounds on the signal reconstruction error of the proposed algorithm. The geometry of the expander graphs makes them provably superior to random dense sensing matrices, such as Gaussian or partial Fourier ensembles, for the Poisson noise model. We support our results with experimental demonstrations.

==> TV.tex <==

\subsection{Approximating the Piecewise-Smooth Signals}
The bounds of Eq.~(\ref{becca}) are valid whenever the signal is
sparse or almost sparse in the canonical basis. This is because the
left hand side of the RIP-1 inequality (\ref{ripeq}) is
only valid for sparse signals. However, since the right hand side of
the inequality is valid for all signals, Eq.~(\ref{measure}) is
always valid, and hence the MAP decoding algorithm with expander
graphs always outputs a signal that is close to the original signal in
the measurement domain. In other words, it removes the Poisson noise
from the compressively sampled signal. If the signal is not sparse in
the measurement domain, there is no general guarantee for exact
recovery of the original signal. However, for signals such as images,
that are piecewise smooth in the canonical basis, we can recover a
sparse approximation of the \textit{gradient} of the signal by
minimizing its \textit{total variance norm}. Define
\begin{equation}
\label{TV}
\|\xb\|_{TV}=\sqrt{\sum_{i,j} (x_{i+1,j}-x_{i,j})^2+(x_{i,j+1}-x_{i,j})^2}.
\end{equation}
Then if a piecewise smooth signal (image) is compressively sampled by
an expander graph, we can approximate it by solving the following min
TV program:
\begin{equation}
  \mbox{minimize }\|\xb\|_{TV}\mbox{  s.t. } \|\Phii \xb-\yb\|_2\leq \delta,
\end{equation}
where $\delta$ is a thresholding function. The min TV approach is
known to be superior to the $\ell_1$ minimization for image recovery
since it avoids the high-frequency artifacts \cite{CRT,berinde}. As a
result, if the image is piecewise smooth, we can first use the MAP
decoding algorithm of Eq.~(\ref{min}) to remove the Poisson
noise, and then use the min TV recovery algorithm to approximate the
original piecewise-smooth signal.

\todo{Sina: we need more here. (1) what is the advantage of this
  two-stage approach over TV-regularized MAP estimation (i.e. using
  Poisson likelihood)? Your email seemed to indicate it was just that
  you could then use off the shelf code instead of writing new code;
  is that all, or is there more? (2) If your claim is that the Poisson
  solution has bounded errors, as you said in your email, then you
  need to state that formally with some supporting argument.}


==> appa.tex <==
\section{Proof of the RIP-1 property}
\label{app:rip}
The upper bound is trivial using the triangle inequality, so we only prove the lower bound.

The left side inequality is not influenced by changing the position of
the coordinates of $x$, so we can assume that they are in a
non-increasing order: $|x_1|\geq |x_2| \geq ... \geq |x_n|$. Let $E$
be the set of edges of $G$ and $e_{ij}=(x_i,y_j)$ be the edge that
connects $x_i$ to $y_j$. Define $$E_2=\{e_{ij}:~
\exists~k<i~\mbox{s.th.}~e_{kj}\in E\},$$ Intuitively $E_2$ is the set
of the collision edges. Let $$T_i=\{e_{i'j}\in E_2~\mbox{s.th.}~i'\leq
i\},$$ and $a_i=|T_i|$.

Clearly $a_1=0$; moreover by the expansion
property of the graph for any $k'$ less than or equal to $k$ $a_{k'}$
is less than or equal to $\epsilon dk'$. Finally since the graph is
$k$-sparse we know that for each $k''$ greater than $k$, $x_{k''}$ is
zero. Therefore
\begin{eqnarray*}
	\sum_{\ei\in E_2} |x_i| &=& \sum_{i=1}^n |x_i|
        (a_i-a_{i-1})\nonumber\\
&=& \sum_{i\leq k} a_i (|x_i|-|x_{i+1}|)\nonumber\\ 
&\leq& \sum_{i\leq k}	\epsilon di (|x_i|-|x_{i+1}|)\nonumber \\ 
&\leq& \sum_{i\leq k} |x_i| \epsilon d = \epsilon d \left\|x\right\|_1. \nonumber
\end{eqnarray*} 
Now the triangle inequality, and the definition of $E_2$ imply
\begin{eqnarray*}
\lefteqn{\left\|Ax\right\|_1}\\
 &=&  \sj \left|\sum_{\ei\in E} x_i\right| = \sj \left|\sum_{\ei \in E_2} x_i + \sum_{\ei \notin E_2} x_i \right |  \nonumber \\
&\geq& \sj \left(\left|\sum_{\ei \notin E_2} x_i\right| - \left|\sum_{\ei \in E_2} x_i \right|\right) \nonumber \\
&=&\sj \left (\left |\sum_{\ei \notin E_2} x_i\right| + \left|\sum_{\ei \in E_2} x_i \right|-2 \left|\sum_{\ei \in E_2} x_i \right| \right) \nonumber \\
 &\geq& \sum_{ \ei \notin E_2} |x_i| +  \sum_{ \ei \in E_2} |x_i | - 2 \sum_{\ei \in E_2} | x_i | \nonumber\\ &\geq& d \left\|x\right\|_1 - 2\epsilon d \left\|x\right\|_1 \nonumber \\ &=& (1-2\epsilon)~d~\|x\|_1 \nonumber. 
\end{eqnarray*} 


\section{Proof of Lemma \ref{l2}}

==> appb.tex <==
\label{nowak}
By Lemma \ref{int} we have
\begin{eqnarray*}
\lefteqn{\Ex_{\Yb|\A\xs}\left[ \sum_{i=1}^m
  \left|(\A\xs)_i^{1/2}-(\A\xh)_i^{1/2} \right|^2 \right]}
\\ \nonumber
&=&\Ex_{\Yb|\A\xs}\left[ 2\log
  \frac{1}{\left(\int{\sqrt{p(\Yb|\A\xs)p(\Yb|\A\xh)}dv(\yb)}
    \right)}\right]. 
\end{eqnarray*}
Clearly \begin{eqnarray*}
\nonumber \lefteqn{\int{\sqrt{p(\Yb|\A\xs)p(\Yb|\A\xh)}dv(\Yb)}} \\ 
\nonumber
&=&\Ex_{\Yb|\A\xs}\left[\sqrt{\frac{p(\Yb|\Phii\xh)}{p(\Yb|\Phii\xs)}}\right].\end{eqnarray*}
We now provide a bound for this expectation. Note that 
\begin{eqnarray}
\nonumber 
\lefteqn{\frac{1}{\longz}}\\ \nonumber &\leq&
\frac{\sqrt{p(\Yb|\A\xh)}e^{-\text{pen}(\xh)}}{\sqrt{p(\Yb|\A\xt)}e^{-\text{pen}(\xt)}\longz}, 
\end{eqnarray}
where $\xt$ is a minimizer in Eq.~(\ref{18}). We can split
the quantity
$$
  2\Ex_{\Yb}\left[\log\left(\frac{\sqrt{p(\Yb|\A\xh)}e^{-\text{pen}(\xh)}}{\sqrt{p(\Yb|\A\xt)}e^{-\text{pen}(\xt)}\longz}\right)\right] 
$$
into three terms:
\begin{eqnarray*}
  \lefteqn{\Ex\left[\log
      \left(\frac{p(\Yb|\A\xs)}{p(\Yb|\A\xt)}\right)\right]+2\text{pen}(\xt)}\\
    \nonumber &+&
    2\Ex\left[\log\left(\frac{\sqrt{p(\Yb|\A\xh)}e^{-\text{pen}(\xh)}}{\sqrt{p(\Yb|\A\xs)}\longz}
      \right)\right]. 
\end{eqnarray*}
We show that the third term is always non-positive, which completes
the proof. Using Jensen's inequality 
\begin{eqnarray*}\nonumber
\lefteqn{\Ex\left[\log\left(\frac{\sqrt{p(\Yb|\A\xh)}e^{-\text{pen}(\xh)}}{\sqrt{p(\Yb|\A\xs)}\longz}
    \right)\right]}\\ \nonumber &\leq&
  \log\left(\Ex\left[\frac{\sqrt{p(\Yb|\A\xh)}e^{-\text{pen}(\xh)}}{\sqrt{p(\Yb|\A\xs)}\longz}
    \right]\right). 
\end{eqnarray*}
Now
\begin{eqnarray*} 
\nonumber
\lefteqn{\Ex\left[\frac{\sqrt{p(\Yb|\A\xh)}e^{-\text{pen}(\xh)}}{\sqrt{p(\Yb|\A\xs)}\longz}
  \right]}
\\ \nonumber &=& \sum_{\xb\in\Gamma} e^{-\text{pen}(\xb)} \frac{\Ex\left[\sqrt{\frac{p(\Yb|\A\xb)}{p(\Yb|\A\xs)}}\right]}  {\longz}
\\ \nonumber &=&  \sum_{\xb\in \Gamma} e^{-\text{pen}(x)}<1.
\end{eqnarray*}

